MASCARA-4 b/bRing-1b - A retrograde hot Jupiter around the bright A3V star HD 85628

In this paper, we aim to characterize a transiting planetary candidate in the southern skies found in the combined MASCARA and bRing data sets of HD 85628, an A3V star of V = 8.2 mag at a distance 172 pc, to confirm its planetary nature. The candidate was originally detected in data obtained jointly with the MASCARA and bRing instruments using a BLS search for transit events. Further photometry was taken by the 0.7 m CHAT, and radial velocity measurements with FIDEOS on the ESO 1.0 m Telescope. High resolution spectra during a transit were taken with CHIRON on the SMARTS 1.5 m telescope to target the Doppler shadow of the candidate. We confirm the existence of a hot Jupiter transiting the bright A3V star HD 85628, which we co-designate as MASCARA-4b and bRing-1b. It is in a 2.824 day orbit, with an estimated planet radius of $1.53 ^{0.07}_{0.04}$ $R_{\rm{Jup}}$ and an estimated planet mass of $3.1 \pm 0.9$ $M_{\rm{Jup}}$, putting it well within the planet mass regime.. The CHAT observations show a partial transit, reducing the probability that the transit was around a faint background star. The CHIRON observations show a clear Doppler shadow, implying that the transiting object is in a retrograde orbit with $|\lambda| = 247.5 \pm 1.6 $\textdegree. The planet orbits at at a distance of 0.047 $\pm$ 0.004 AU from the star and has a zero-albedo equilibrium temperature of 2100 $\pm$ 100 K. In addition, we find that HD 85628 has a previously unreported stellar companion star in the Gaia DR2 data demonstrating common proper motion and parallax at 4.3 arcsecond separation (projected separation $\sim$740 AU), and with absolute magnitude consistent with being a K/M dwarf.

==> Unused.tex <==

 These systems are good candidates for atmospheric characterization, and can be used to detect the presence of species with large cross sections but smaller abundances such as TiO, VO, and alkali metals, which are expected to be present in hot, highly irradiated planets ($T_{eq} >2000K$), and could be a cause of inversion layers (\cite{MadhusudhanSeager2009}). These elements  have been detected in planets such as HD209458b (\cite{Desert2008A&A...492..585D}), WASP33-b (\cite{Nugroho2017AJ....154..221N}), and WASP19-b (\cite{Sedaghati2017Natur.549..238S}). 

Observations with high resolution spectrographs during a planet transit on a high magnitude star, when coupled with detailed atmospheric models, can constrain many atmospheric properties ranging from the temperature structure, and the composition and presence of clouds and hazes (\cite{MadhusudhanSeager2009}, \cite{Sing2012}, \cite{Dressing2015}), which is not as easily done on fainter targets due to photon noise. Shorter period planets make it easier to coordinate for observation time. As such, higher magnitude, shorter period stars are excellent candidates for followup studies.


It is for these reasons that NASA has launched the Transiting Exoplanet Survey Satellite (TESS) (\cite{TESS_main}) in 2018. TESS is a space-based observatory that is able to identify a wide range of planets (from super-Earths to hot Jupiters) orbiting a wide range of stellar types for a wide range of orbital distances (\cite{Tess_ExoplanetPredictions}). TESS has already released data products for sectors 1-5 (observing almost one half of the southern hemisphere), and will be finished observing the southern hemisphere in mid-2019. TESS is expected to observe MASCARA-4 b in sector 9, which will be useful in constraining its transit behind the host star. Other ground-based observatories probing the brighter end of systems includes the Kilo-degree Extremely Little Telescope (KELT) survey (\cite{KELT2007PASP..119..923P}), operational since 2005 in the northern hemisphere and since 2009 in the southern hemisphere.


In this paper we will describe the discovery of MASCARA-4 b/bRing-1 b, henceforth referred to as MASCARA-4 b. This planet is a joint discovery between the Multi-Site All-Sky CAmeRA (MASCARA) (\cite{MASCARA_instrument}) and bRing (\cite{bRing_instrument}). This planet is the fourth planet discovered by MASCARA, which has previously found MASCARA-1 b (\cite{MASCARA_science_1}), MASCARA 2-b (\cite{MASCARA_science_2}), and MASCARA 3-b (\cite{MASCARA_Science3}), and is the first planet discovered by bRing, which has previously been used to discover $\delta$ Scuti pulsations in HD 156623 (\cite{Mellon2019}). MASCARA-4 b orbits the star HD 85628, a bright ($V_{mag}=8.2$) A3V star with a dim binary companion. In Section \ref{Sec: Discovery_Obs} we describe the discovery observations performed by the MASCARA and bRing network. Section \ref{Sec: Followup} describes the followup observations performed by CHAT, FIDEOS, and CHIRON. Section \ref{Sec: Parameters_Analysis} presents the full analysis of the system parameters of MASCARA-4 b, which are discussed in Section \ref{Sec:Discussion}.

%Discuss the system here
 Of particular note for MASCARA-4 b is the planets retrograde motion with respect to its host star. While a large fraction of Hot Jupiters ($>40\%$) show significant misalignment with respect to their host star orbit (\cite{Albrecht2012}), now only fourteen planets are known to orbit in a retrograde motion (\cite{tepcet2011MNRAS.417.2166S}), meaning that the inclination of the planet is between $-5\pi/8$ to $-11\pi/8$ or $5\pi/8$ to $11\pi/8$. It is currently unknown exactly how such an extreme spin-orbit misalignment comes to be, but some explanations include secular mutual close encounters, or through Kozai-Lidov oscillations, where the orbital eccentricity and inclination of the hot Jupiter changed due to the influence of a distant companion. This causes an orbit that can be significantly tilted with respect to the orbit of the inner planet (\cite{Naoz2011}, \cite{Nagasawa2008}). MASCARA-4 b is around the brightest known star with a retrograde planet, with a visual magnitude of 8.2.









%RV
, along with the measurement of precision radial velocities and bisector spans using the cross-correlation technique. From these spectra we identified that MASCARA-4 has a moderately high rotational velocity (vsini $\approx$ 45 km s$^{-1}$), which was expected given its spectral type. Even though, the limited precision of the radial velocity measurements due to this rapid rotation was not enough to measure RV variations produced by a planetary mass companion, they were useful to reject the presence of stellar companions that could have been responsible for the transits.



%Stellar parameters

The {\it Stilism} 3D interstellar reddening map \citep{Lallement14, Capitanio17}
shows that the predicted reddening at the position of the HD 85628 system is small, 
but non-zero: {\it E(B-V)} = 0.020\,$\pm$\,0.018 mag, or for a standard interstellar
extinction law \citep[e.g.]{Olson75}: extinction $A_V$ = 0.066\,$\pm$\,0.059 . 
%
The $B-V$ color for HD 85628 A \citep[0.200\,$\pm$\,0.013;][]{ESA97} is somewhat
redder than for the mean B-V for stars classified by Houk as A3V (mean $B-V$ = 0.14),
suggesting that the reddening could be as high as E($B-V$) $\simeq$ 0.06. 




%Discussion
, one of only 14 retrograde Hot Jupiters known to date (joining WASP-2\,b, WASP-8\,b, WASP-15\,b, WASP-17\,b, WASP-60\,b, WASP-94A\,b, WASP-167\,b \citep{WASP2b15b17b}, \citep{WASP8b2010A&A...517L...1Q}, \citep{GAPS_Survey2018}, \citep{WASP942014A&A...572A..49N}, \citep{WASP167b_2017MNRAS.471.2743T}, HAT-P-6\,b, HAT-P-7\,b, HAT-P-14\,b, HAT-P-18\,b \citep{HATP6b2011A&A...527L..11H}, \citep{HATP7b2009ApJ...703L..99W}, \citep{HATP14b2011AJ....141...63W}, \citep{HATP18b2014A&A...564L..13E}, KELT-17\,b, and KELT-19\,b \citep{KELT17b2016AJ....152..136Z}, \citep{KELT19b2018AJ....155...35S} and its host star is the brightest star with a retrograde planet known currently.
